Domain Adaptation from Scratch

Natural language processing (NLP) algorithms are rapidly improving but often struggle when applied to out-of-distribution examples. A prominent approach to mitigate the domain gap is domain adaptation, where a model trained on a source domain is adapted to a new target domain. We present a new learning setup, ``domain adaptation from scratch'', which we believe to be crucial for extending the reach of NLP to sensitive domains in a privacy-preserving manner. In this setup, we aim to efficiently annotate data from a set of source domains such that the trained model performs well on a sensitive target domain from which data is unavailable for annotation. Our study compares several approaches for this challenging setup, ranging from data selection and domain adaptation algorithms to active learning paradigms, on two NLP tasks: sentiment analysis and Named Entity Recognition. Our results suggest that using the abovementioned approaches eases the domain gap, and combining them further improves the results.

==> Eyal_Yftah - Active Learning for unsupervised DA/1.intro.tex <==


\section{Introduction}
\label{sec:intro}

% \item NLP algorithms are the best thing ever!!! But they need annotated data:).
Natural Language Processing (NLP) algorithms have made impressive progress in recent years, achieving great success in various tasks and applications. However, these algorithms may require substantial labeled data to reach their full potential. Such data is often too costly and labor-intensive to obtain. Furthermore, modern systems are required to perform well on data from many domains, while for most tasks, labeled data is available for only a few. Consequently, NLP algorithms still struggle when applied to test examples from unseen domains \citep{dilbert, pada, docogen}. 

% \item The general procedure for annotating data is through crowd sourcing. However, when the data in hand is sensitive: medical. virtual assistant, military applications, etc. crowdsourcing is not sn option.  Talk about privacy and why some organizations can not label data of interest via online annotation platforms, e.g., smart assistant - recording customers, military applications, etc. Therefore the cost of annotating directly from the distribution of interest is too high. In this paper, we examine what one can do when examples from the target distribution can not be obtained, but obtaining annotated examples from available domains are costly.
A common strategy for annotating data is through crowdsourcing platforms, e.g., Amazon Mechanical Turk, where data can be annotated on a large-scale, as one can harness a large workforce at affordable prices. However, crowdsourcing is not an option for sensitive data (e.g., in medical and military applications). For instance, virtual assistants such as Alexa, Siri, and Google Home serve millions of users. Annotating data from virtual assistants' recorded conversations would be optimal input for training applicable NLP models for their purposes. However, crowdsourcing is not a valid option for such sensitive data as it does not preserve users' privacy. Hiring annotators internally is expensive and often hard to scale efficiently.  

This paper examines different approaches to annotating and using data from non-sensitive sources (NSS) when \emph{target domain data can not be annotated}. More precisely, we experiment with several methods (\S\ref{sec:methods}) to train a model for a sensitive target domain under a given annotation budget of examples from NNS. Various methods aim to ease the burden of data annotation. 
For example, domain adaptation (DA) algorithms are trained on source domain training data to be effectively applied to other target domains. 
% For example, in domain adaptation (DA) a model is trained on source domain training data so that it can be effectively applied to other target domains. 
% For example, Domain Adaptation (DA), training a model using source domain labeled data and applying it effectively to a target domain. 
% DA is a vast field of research, varying in the amount of target domain supervision availability. 
Several setups have been explored in the DA literature,  differing in the availability of target domain supervision. 
This paper focuses on unsupervised DA (UDA), i.e., where no labeled data is available from the target domain. Still, unlabeled data can be freely obtained from both source and target domains. Unlike previous works on UDA \cite{ziser-pblm, perl}, trying to train the best model for a given labeled source data, we are interested in efficiently annotating the source data. Hence, we perform domain adaptation from scratch. 

%Thus, the go-to option is to annotate exterior data. Can this be done intelligently: Should the bank prioritize specific domains for annotation on others or optimally select out-of-domain examples given the target domain? This paper examines what one can do when labeled examples from the target distribution can not be obtained, and obtaining annotated examples from available source domains is costly.  

% \item Talk about domain adaptation. DA algorithms can address the aforementioned issues by applying an algorithm trained on annotated data from several source domains to data that arrives from sensitive target domains. 





% \item Talk about active learning
Another prominent approach for coping with limited annotation resources is  Active Learning (AL, \citep{DBLP:journals/jair/CohnGJ96}). AL algorithms automatically choose a subset of unlabeled samples from a massive unlabeled corpus, maximizing the value of the labeling process. Such algorithms have shown effectiveness for deep neural network (DNN) modeling across various NLP tasks \citep{DBLP:conf/acl/DuongAEPCJ18, DBLP:conf/conll/PerisC18, DBLP:conf/emnlp/Ein-DorHGSDCDAK20}. 
% AL algorithms choose 
The typical assumption in the AL literature is that AL algorithms choose the most valuable subset to annotate under the assumption of being tested on data from the same distribution. This paper examines their usefulness in improving model performance when applied to unknown target domains. 
% in improving the results for a different domain from the one they applied to. 

As DA and AL are highly popular approaches to ease the problem of insufficient annotation budget, combining the two is natural \cite{rai2010domain, saha2011active}. 
% Most previous works 
Most works in this intersection share a similar setup, in which labeled data from a source domain facilitates the annotation process in the target domain \citep{li2013active, wu2017active}.
% \citet{li2013active} train classifiers for the source and  target domains (one per each) and annotate the lowest certainty samples out of the examples on which the classifiers disagree. 
% \citet{wu2017active} acquire labeled data from the target domain to adapt general-purpose sentiment lexicons. Together with similarities among source and target domain-specific words, they train a sentiment analysis classifier.
% \citet{wu2017active} use hand-crafted rules and concurrence statistics to obtain sentiment similarities
% among source and target domain-specific words. Combined with AL-acquired labeled data from the target domain, these similarities are used to train a sentiment analysis classifier for the target domain. 
\citet{xiao2013online} consider 
% a setup where 
data annotation to be cheaper in the source domain compared to the target domain.
% , while in both it is costly. 
% They iteratively obtain two samples, one from the source domain and one from the target domain. The probability of choosing one sample over the other is directly driven by the annotation cost of its corresponding domain. 
% They iteratively obtain two samples, one from each domain, and set the probability of choosing one sample over the other directly by the domain annotation cost. 
% Then, if the sample meets an uncertainty condition, it is sent for human annotation. 
% While annotating samples from the target domain is not available in our setup, we consider this work the most similar to ours since it recognizes the cost of annotating samples from the source domain for performing well in the target domain.
We consider this work the most similar to ours since it recognizes the cost of annotating samples from the source domain for improving in the target domain. However, annotating samples from the target domain is unavailable in our setup.

% \item Talk about the intersection between the two (you can find it here \url{https://docs.google.com/document/d/1CTrUVDrCHGIMHDq3f16AsDo2VPrFPcTAEZ3id9jneio/edit}) and say that in this works the tagging is done in the target domain.
%Few works have looked into the intersection of AL and DA in NLP, mainly focusing on annotating examples from a target domain \citep{}. This work investigates a new setting in which target domain data cannot be annotated. Concretely, we assume the availability of unlabeled data from multiple source and target domains and aim to label the source domain examples that will maximize the model's performance on data from the target domain.  To the best of our knowledge, this work is the first to tackle this challenging setup within the intersection of DA and AL.



% \item Talk briefly about the results:
% \item PAD
% \item weakly supervised DA 
% \item PAL-PERL
% \item Active learning seems to work better on NLP tasks with a structured output, even in the DA setup.
%We perform extensive experimentation in the proposed scenario, where source domain data annotation is costly, and target domain data annotation can not be obtained. To this end, we consider two prominent NLP tasks, sentiment analysis and named entity recognition. We first present the performance of SOTA sentiment classification algorithms for low resource UDA, introducing an unsupervised technique for selecting the initial examples for low resource UDA. We then experiment with three types of AL techniques in the proposed setting: (1) traditional AL techniques; (2) general DA techniques integrated into the AL scheme; and (3) task-specific DA algorithms adapted to AL. Based on our extensive experimentation, we provide a comprehensive perspective on the pros and cons of each of the proposed techniques.  Finally, we introduce a new pivot-based AL technique for sentiment classification and show that it is better to limit the AL algorithm to specific sources given a target domain. We also introduce a method for finding these source domains.       

We propose and evaluate various methods to tackle the challenging ``DA from scratch'' setup, focusing on two tasks: Binary sentiment classification and named entity recognition. 
Going beyond existing methods, we propose several methods for integrating domain knowledge into AL systems and demonstrate encouraging results:  Combining the two is better than applying them separately. We hope to inspire future work in this direction. 






==> Eyal_Yftah - Active Learning for unsupervised DA/2.problem-definition.tex <==



\section{Problem Definition}
\label{sec:problem}
The goal of a DA algorithms is to learn a model $m$ that generalizes well from a set of source domains  $\{\mathcal{D}_{S_i}\}_{i=1}^{K}$ to a  target domain $\mathcal{D}_T$, for a given task. 
We assume that unlabeled data from the source and target domains are available. 
% We denote them 
We denote the corresponding unlabeled sets with $\{\mathcal{U}_{S_i}\}_{i=1}^{K}$  and $ \mathcal{U}_T $ respectively. Initially, no labeled data exists, and since data from the target domain is sensitive, we cannot annotate it. Thus, we consider an approach for automatically choosing  $L$ source domain examples to annotate in each iteration. We choose examples that would best benefit a model applied to test data that originates from the target domain.  

\begin{table}
\small
\centering
\begin{adjustbox}{width=0.35\textwidth}

\begin{tabular}{| l | l | c | c | c | c | c|}
\hline
  & & \multicolumn{4}{c|}{Method} \\
   Section & Name  & \multicolumn{1}{c}{\rotatebox[origin=c]{90}{\tiny{DA}}} & \multicolumn{1}{c}{\rotatebox[origin=c]{90}{\tiny{AL}}}  & \multicolumn{1}{c}{\rotatebox[origin=c]{90}{\tiny{NIS}}} &\rotatebox[origin=c]{90}{\tiny{DS}} \\
\hline

\multirow{1}{*}{\S\ref{sec:naive}} &\rbert & \xmark  &  \xmark  & \xmark & \xmark \\
\hline

\multirow{3}{*}{\S\ref{sec:basic-al}} &\bert & \xmark &  \cmark   & \xmark & \xmark \\
&\dropout & \xmark  & \cmark & \xmark &  \xmark \\
&\smoothing & \xmark &   \cmark  & \xmark & \xmark \\
\hline

\multirow{2}{*}{\S\ref{sec:da-no-al}} &\rdt & \cmark &   \xmark  & \xmark & \xmark \\
&\rdann & \cmark &  \xmark  & \xmark & \xmark \\
\hline

\multirow{2}{*}{\S\ref{sec:iterative-certainty}} &\dt & \cmark &  \cmark   & \xmark & \xmark \\
&\dann & \cmark &   \cmark  & \xmark & \xmark \\
\hdashline

\multirow{3}{*}{\S\ref{sec:domain-similarity}} &\select & \cmark &   \cmark  & \cmark & \xmark \\
&\rtapad & \cmark &  \xmark  & \xmark & \cmark \\
&\tapad & \cmark &  \cmark   & \xmark & \cmark \\


\hline
\end{tabular}
\end{adjustbox}
\caption{Our methods. We specify which use domain adaptation (DA), active learning (AL), non-iterative example selection (NIS), and domain selection (DS).}
\label{tab:methods}
\end{table}


==> Eyal_Yftah - Active Learning for unsupervised DA/3.methods.tex <==






\section{Methods}
\label{sec:methods}

Table~\ref{tab:methods} outlines our methods, which are divided into four branches: (1) Supervised learning with naive labeling (\S\ref{sec:naive}); (2) active learning methods (\S\ref{sec:basic-al}); (3) domain adaptation approaches (\S\ref{sec:da-no-al}); and (4) methods that combine domain adaptation with  AL (\S\ref{sec:DA-and-AL}).\footnote{There are two folk wisdom definitions of AL. The first clings to sample selection while the second advocates interactivity. For simplicity, we follow the first definition.} 
% We next elaborate on each of these branches.
% , specifying the experimented models for each solution.
We implement all our algorithms with a pretrained BERT model \citep{bert}.
% We apply all presented algorithms on BERT \citep{bert}.


\subsection{Supervised Learning with Naive Labeling}
\label{sec:naive}
% To demonstrate how challenging our proposed setup is,
We first apply a straightforward approach. 
Particularly, we randomly choose which examples to annotate and finetune an out-of-the-box BERT on the labeled data. We name this baseline \textbf{\rbert}. 



% no domain adaptation
\subsection{Active Learning Approaches}
\label{sec:basic-al}
% Although we present a challenging setting which incorporates domain adaptation and active learning, a potential (naive) solution could be implementing an algorithm that neglects the DA idea. 
We implement a set of algorithms that perform example annotation according to the model's certainty. We test the following models: (a) \textbf{\bert}, iteratively choosing examples according to the (in)confidence of a BERT trained on the available annotated examples (so far); (b) \textbf{\dropout} (\textit{monte-carlo dropout}, \citep{DBLP:conf/icml/GalG16}), applying many dropout instances of the example to get a more robust certainty score of the model; and (c) \textbf{ \smoothing} (\textit{label smoothing}), a variant of \bert{}  but when the underlying NLP model is trained with a label smoothing objective.


\begin{figure}

\begin{minipage}{.48\textwidth}
\centering
\includegraphics[scale=.33]{figures/plot_bar.png}
\end{minipage}

\begin{minipage}{.24\textwidth}
\centering
\subfloat[\textbf{DVD}]{\label{fig:dvd}\includegraphics[scale=.18]{figures/blitzer/DVD-graph.png}}
\end{minipage}%
\begin{minipage}{.24\textwidth}
\centering
\subfloat[\textbf{Electronics}]{\label{fig:electronics}\includegraphics[scale=.18]{figures/blitzer/electronics-graph.png}}
\end{minipage}

\begin{minipage}{.24\textwidth}
\centering
\subfloat[\textbf{BC}]{\label{fig:bc}\includegraphics[scale=.18]{figures/NER/BC-graph.png}}
\end{minipage}%\par\medskip
\begin{minipage}{.24\textwidth}
\centering
\subfloat[\textbf{NW}]{\label{fig:nw}\includegraphics[scale=.18]{figures/NER/NW-graph.png}}
\end{minipage} \par\medskip
\caption{Sentiment classification (a-b) and NER (c-d) results with a breakdown to active learning iteration.}
\label{fig:sa-ner-main}
\end{figure}


\subsection{Domain Adaptation}
\label{sec:da-no-al}
UDA algorithms require unlabeled data from the source and target domains and labeled data only from the source domain, to be applied to test data from the target domain. 
We implement two popular UDA algorithms: (1) \textbf{\rdt} (\textit{domain-tuned} \citep{DBLP:conf/emnlp/HanE19}), which is first finetuned on the available unlabeled data (from the source and target domains) by performing the language modeling task.
% \footnote{Since we use BERT, we use the masked language modeling objective \citep{bert}.} 
Then, it is further finetuned on task labeled data from the source domains; (2) \textbf{\rdann}  (\textit{domain adversarial neural networks} \citep{dann}), a model that integrates BERT with an adversarial domain classifier to learn domain invariant representations. \rdann{} performs multi-task training, combining the downstream task and the adversarial objectives. 
For both methods, we randomly select the source domain examples for annotation.
% , as we do not perform AL.
% task independant Domain adaptation (model agnostic active learning)
\subsection{Combining DA and AL}
\label{sec:DA-and-AL}
We next introduce novel approaches for incorporating DA methods within AL algorithm. We distinguish between iterative and non-iterative example selection  methods (IS and NIS). 
Finally, we present a domain-selection (DS) method, choosing a single source domain to represent the annotation pool.



\subsubsection{Iterative Certainty-based Algorithms}
\label{sec:iterative-certainty}
We present \textbf{\dt{}} and \textbf{\dann}, UDA models corresponding to the ones described in \S\ref{sec:da-no-al} and combined with \bert. Unlike \rdt{} and \rdann, where the source domain annotated examples are randomly selected, these models train on labeled data iteratively selected by their confidence scores.








% We follow a straightforward technique to apply the UDA algorithms presented in \S\ref{sec:da-no-al} within the AL process. 
% We apply the UDA algorithms presented in \S\ref{sec:da-no-al} experiment two prominent DA algorithms which take advantage of the large amount of unlabeled data from source and target domains: (1) \textbf{Domain-tuned BERT (\dt)}, which is finetuned on the available unlabeled data (from source and target domains) by performing the language modeling task.\footnote{Since we use BERT, this is performed with the masked language modeling objective \citep{bert}.} After this additional finetuning step, the model performs the AL paradigm; (2) \textbf{domain adversarial neural networks (\dann)}, a model that integrates \bert with an adversarial domain classifier to learn domain invariant representations. \dann performs multi-task training, combining the downstream task and the adversarial objectives while performing AL iterations.




\subsubsection{Leveraging Domain Similarities}
\label{sec:domain-similarity}

Utilizing domain-similarity metrics 
to select the most adaptable examples for annotation,  lies at the intersection
% to select the most adaptable samples lies in the intersection 
of AL and DA. $A-$distance \citep{DBLP:conf/vldb/KiferBG04} is a standard metric for measuring similarity between domains. \citet{ben2007analysis} interpret the \textit{proxy $A-$distance (PAD)} between two domains as the loss a linear classifier achieves when predicting the origin domain of samples obtained from both domains. As PAD is task-independent, it can not harness any information about the task at hand. To address this problem, \citet{elsahar2019annotate} introduced the  \textit{task-adapted Proxy $A-$distance} (TAPAD)\footnote{\citet{elsahar2019annotate}  named this measure PAD*.} measure, which trains the domain-discrimination model on representations obtained from a model which is finetuned for a downstream task. TAPAD has been demonstrated to effectively predict the performance degradation for cross-domain setups.







\paragraph{Task-adapted Proxy $A-$distance (TAPAD) }
We propose a novel integration of TAPAD as part of an AL mechanism. After randomly sampling the initial annotation seed, we train a model for the downstream task. Then, we tune the model for discriminating between source and target examples, using unlabeled data from the source and target domains. We then measure the TAPAD score between each of the source domains and the target domain.  Finally, we constrain the annotation pool to contain data only from the most similar source domain for the rest of the annotation process. 
We implement two methods for selecting the data for annotation from the most similar domain: either randomly, with \textbf{\rtapad}, or using an uncertainty measure, with \textbf{\tapad}.

\paragraph{Non-iterative Example Selection}
We implement a domain discriminator trained on unlabeled data from the source and target domains. The predictor is then used to provide a score $\mathcal{S}(x)$ for each example ($x$, from the source domains), where  $\mathcal{S}(x) = \frac{1}{M(x)}$ and $M(x)$ is the predictor's output. The model scores range from $0$ to $1$, higher scores mean the model is more confident that the example
originates from the corresponding source domain.
% arrives from a source domain. 
We annotate the top $L$ ranked unlabeled examples. 
% We sort the unlabeled examples by their scores and annotate the top $L$. 
Since the scores are not affected by new annotations, we do not need to re-rank the examples iteratively. We name this algorithm \textbf{\select}. 







  


==> Eyal_Yftah - Active Learning for unsupervised DA/4.experimental-setup.tex <==



\begin{table*}

\centering
\begin{adjustbox}{width=0.87\textwidth}

\begin{tabular}{ | l || c | c | c | c | c || c || c | c | c | c | c | c || c |}
\hline
& \multicolumn{6}{c||}{\textbf{Sentiment}} & \multicolumn{7}{c|}{\textbf{NER}} \\ 
\hline
  & \textbf{A}  & \textbf{B} & \textbf{D} & \textbf{E} & \textbf{K} & \textbf{AVG}  & \textbf{BC}  & \textbf{BN} & \textbf{MZ} & \textbf{NW} & \textbf{TC} & \textbf{WB} & \textbf{AVG}  \\
\hline

\textbf{\rbert} & $ 77.0 $ &  $ 75.0 $ & $ 72.3 $ & $ 76.0 $ & $ 78.1 $ & $ 75.4 $ & $ 46.5 $ &  $ 48.5 $ & $ 42.1 $ & $ 36.2 $ & $ 32.5 $ & $ 30.7 $ & $ 39.4 $  \\
\hline
\textbf{\bert}     & $ 75.8 $ &  $ 75.7 $ & $ 73.7 $ & $ 76.2 $ & $ 76.7 $ & $ 75.3 $ & $ 50.9 $ &  $ 55.1 $ & $ 45.2 $ & $ 47.1 $ & $ 32.8 $ & $ 34.1 $ & $ 44.2 $  \\
\textbf{\smoothing}     & $ 75.1 $ &  $ 74.7 $ & $ 75.3 $ & $ 77.1 $ & $ 77.6 $ & $ 76.0 $ & $ 51.4 $ &  $ 55.7 $ & $ 47.0 $ & $ 48.8 $ & $ 33.8 $ & $ 33.7 $ & $ 45.1 $  \\
\textbf{\dropout}     & $ 76.7 $ &  $ 72.9 $ & $ 72.7 $ & $ 79.0 $ & $ 79.8 $ & $ 76.2 $ & $ 51.1 $ &  $ 54.8 $ & $ 43.7 $ & $ 46.7 $ & $ 32.5 $ & $ 33.6 $ & $ 43.7 $  \\
\hline
\textbf{\rdt}   & $ \textbf{78.0} $ &  $ 78.1 $ & $ 76.2 $ & $ 79.5 $ & $ 82.1 $ & $ 78.6 $ & $ 47.7 $ &  $ 51.0 $ & $ 43.0 $ & $ 38.4 $ & $ 33.8 $ & $ 30.8 $ & $ 40.8 $  \\
\textbf{\rdann} & $ \textbf{78.0} $ &  $ 75.7 $ & $ 77.0 $ & $ 79.5 $ & $ 79.4 $ & $ 77.9 $ & $ 45.9 $ &  $ 46.5 $ & $ 40.4 $ & $ 35.7 $ & $ 32.0 $ & $ 29.1 $ & $ 38.2 $  \\
\hline
\textbf{\dt}       & $ \textbf{78.0} $ &  $ 77.5 $ & $ 77.6 $ & $ 81.2 $ & $ 81.9 $ & $ 79.0 $ & $ 53.2 $ &  $ \textbf{56.3} $ & $ 46.6 $ & $ 48.0 $ & $ 34.4 $ & $ \textbf{34.1} $ & $ 45.4 $  \\
\textbf{\dann}     & $ 75.0 $ &  $ 76.8 $ & $ 77.2 $ & $ 77.8 $ & $ 80.8 $ & $ 77.5 $ & $ 50.9 $ &  $ 54.6 $ & $ 45.9 $ & $ 47.3 $ & $ 32.3 $ & $ 33.2 $ & $ 44.0 $  \\
\hline
\textbf{\select}       & $ 76.9 $ &  $ \textbf{79.7} $ & $ \textbf{82.8} $ & $ \textbf{87.0} $ & $ \textbf{87.0} $ & $ \textbf{82.7} $ & $ 40.2 $ &  $ 48.2 $ & $ 40.9 $ & $ 43.1 $ & $ 12.8 $ & $ 28.4 $ & $ 35.6 $  \\
\textbf{\rtapad}       & $ 77.6 $ &  $ 76.5 $ & $76.2 $ & $ 82.2 $ & $ 80.9 $ & $ 78.7 $ & $ 50.2 $ &  $ 50.3 $ & $ 45.9 $ & $ 48.7 $ & $ 31.2 $ & $ 26.3 $ & $ 42.1 $  \\
\textbf{\tapad}       & $ 76.9 $ &  $ 74.5 $ & $ 78.1 $ & $ 81.5 $ & $ 80.6 $ & $ 78.3 $ & $ \textbf{55.5} $ &  $ 54.7 $ & $ \textbf{49.4} $ & $ \textbf{53.7} $ & $ 33.2 $ & $ 30.4 $ & $ \textbf{46.2} $  \\
\hline

\hline
\end{tabular}
\end{adjustbox}
\caption{AUC - SA (up to 250 examples) and NER (up to 2500 examples).}
\label{tab:main-results}
\end{table*}




\section{Experimental Setup}
We focus on two common NLP tasks, (binary) sentiment analysis (SA) and named entity recognition (NER). For SA, 
following a large body of prior work \citep{ziser-reichart-2018-deep, ziser19, perl}, 
we include 
% five different domains: 
four product review domains \citep{blitzer2007biographies} - Books (B), DVDs (D), Electronics (E) and Kitchen appliances (K); and an additional airline review dataset (A,  \cite{Nguyen2015airline}).
For NER, we experiment with the OntoNotes 5.0 dataset \citep{ontonotes}, including six different domains: Broadcast Conversations (BC), Broadcast News (BN), Magazine (MZ), Newswire (NW), Telephone Conversation (TC), and Web (WB). We report the statistics of our experimental setups in \S\ref{sec:implementation}.\footnote{URLs of the datasets, code, implementation details, and hyperparameter configurations are described in \S~\ref{sec:implementation}.
}

% We experiment in a leave-one-out fashion, choosing
% We choose a single target domain that is held out during training and is used only for testing. Accordingly, all other domains form our source domains and are used for training. We repeat the experiments in each task to use each domain as the target domain.
% We experiment in a leave-one-out fashion, choosing 
We choose a single target domain that is held during training and used only for testing. Accordingly, all other domains form our source domains and are used for training. We repeat the experiments in each task to use each domain as the target domain.
We start each IS algorithm by randomly sampling $M$ examples and annotating them ($M=50$ and $M=250$ for SA and NER, respectively). Afterward, we choose $M$ examples to annotate in each iteration according to the method in use. 
We report accuracy scores for sentiment classification\footnote{We use balanced test sets for sentiment analysis.} and macro-F1 scores for NER. All reported scores are averaged across five different seeds. To conclude the accumulated results across different iterations, we report the AUC score for each model. 

% \paragraph{Experimental Protocol }
% % \eyal{Describe the setting - separate to tasks.}
% We perform active learning (AL) in a challenging unsupervised domain adaptation (UDA) setting. We follow a many-to-one experimental protocol, in which we choose a single target domain that is held out during training and is used only for testing (for each experiment). Accordingly, all other domains form our source domains and are used for training. At the beginning of each experiment, we build an annotation pool comprised of all labeled examples available in our source domains.  We start the AL algorithm by randomly sampling $M$ examples and annotating them ($M=50$ and $M=250$ for SA and NER, respectively). Afterward, we choose $M$ examples to annotate in each AL iteration according to the method in use. For UDA algorithms (\dt{}, \dann, and \tapad), we use unlabeled data available from all domains (source and target). For NER, where we don't have unlabeled data, we simply use the raw text that is available from the training data of each domain.  






% \paragraph{Models}
% % \eyal{talk about models}
% As described in \S~\ref{sec:methods}, we evaluate several type of solutions for the presented setting, with a total of eleven different algorithm tested on two tasks, SA and NER. We consider three general active learning algorithms \textbf{\bert}, \textbf{\dropout}, and \textbf{\smoothing}, as well as  a non AL benchmark, \textbf{\rbert}. Additionally, we evaluate algorithms that integrate active learning and domain adaptation approaches: (1) \textbf{\dt{}} and \textbf{\rdt}, which are first finetuned on unlabeled data (from the source and target domains) following the LM objective, and then use model-(un)certainty and randomness (no AL) for iterative data selection; (2) \textbf{\dann{}} and \textbf{\rdann{}} (based on uncertainty and randomness, respectively), integrating an adversarial classification head which predicts the example domain; (3) \textbf{\select}, that performs non-iterative data selection according to the in-confidence of a domain discriminator; and (4) \textbf{\tapad} and \textbf{\rtapad}, which first reduce the annotation pool to include only data from a single source domain (according to the TAPAD scores) and then applies \bert{} and \rbert, respectively.      





==> Eyal_Yftah - Active Learning for unsupervised DA/5.results.tex <==

\section{Results and Analysis}
\label{sec:results}








% \hline
% \end{tabular}
% \end{adjustbox}
% \caption{Blitzer - 50 training examples - std.}
% \label{tab:human-intrinsic}
% \end{table}

% \begin{table}
% % \small
% \centering
% \begin{adjustbox}{width=0.45\textwidth}

% \begin{tabular}{ | l || c | c | c | c | c || c |}

% \hline
%   & \textbf{A}  & \textbf{B} & \textbf{D} & \textbf{E} & \textbf{k} & \textbf{AVG}  \\
% \hline
  
% \textbf{BERT} & $ 63.8 $ &  $ 57.7 $ & $ 58.1 $ & $ 60.1 $ & $ 62.1 $ & $ 60.4  $ \\
% \textbf{DANN} & $ 67.8 $ &  $ 66.3 $ & $ 71.5 $ & $ 64.1 $ & $ 69.3  $ & $ 67.8 $ \\
% \textbf{DT} & $ 68.1 $ &  $  60.3 $ & $ 62.8 $ & $ 63.0 $ & $ 67.6 $ & $ 64.4  $ \\
% \textbf{PERL} & $ 82.8 $ &  $ 80.4 $ & $ 81.7 $ & $ 85.8 $ & $ 86.8 $ & $ 83.5 $ \\
% \textbf{Smart-PERL} & $ \textbf{83.3} $ &  $ 82.6 $ & $ 82.6 $ & $ \textbf{86.1} $ & $ \textbf{88.0} $ & $ 84.5 $ \\
% \textbf{Smart-PERL-2} & $ 82.1 $ &  $ \textbf{84.6} $ & $ \textbf{83.9} $ & $ 85.6 $ & $ 87.0 $ & $ \textbf{84.6} $ \\
% \textbf{Smart-PERL-3} & $ 83.0 $ &  $ 80.7 $ & $ 82.7 $ & $ 85.3 $ & $ 86.3 $ & $ 83.6 $ \\
% \hline
% \textbf{UB - 1000 ex} & $ 83.5 $ &  $ 84.6 $ & $ 85.6 $ & $ 90.1 $ & $ 90.8 $ & $ 86.9 $ \\

% \hline
% \end{tabular}
% \end{adjustbox}
% \caption{Blitzer - 50 training examples.}
% \label{tab:human-intrinsic}
% \end{table}





% \begin{table}

% \centering

% \begin{adjustbox}{width=0.45\textwidth}
% \begin{tabular}{ | l || c | c | c | c | c || c |}

% \hline
%   & \textbf{A}  & \textbf{B} & \textbf{D} & \textbf{E} & \textbf{k} & \textbf{AVG}  \\
% \hline
  
% \textbf{BERT-rnd} & $ 82.3 $ &  $ 83.2 $ & $ 83.5 $ & $ 87.7 $ & $ 89.0 $ & $ 85.1 $ \\
% \textbf{BERT-rnd-pad} & $ \textbf{82.8} $ &  $ 84.2 $ & $ 84.4 $ & $ 88.1 $ & $ \textbf{89.9} $ & $ 85.9 $ \\
% \textbf{BERT} & $ 81.2 $ &  $ 83.7 $ & $ 83.3 $ & $ 87.1 $ & $ 87.6 $ & $ 84.6 $ \\
% \textbf{BERT-pad} & $ 82.1 $ &  $ \textbf{84.2} $ & $ \textbf{84.6} $ & $ \textbf{89.5} $ & $ 89.4 $ & $ \textbf{86.0} $ \\

% \hline
% \end{tabular}
% \end{adjustbox}
% \caption{Sentiment - AUC - up to 1000 examples}\label{tab:sentiment-auc}

% \bigskip

% \begin{adjustbox}{width=0.48\textwidth}
% \begin{tabular}{ | l || c | c | c | c | c | c || c |}

% \hline
%   & \textbf{BC}  & \textbf{BN} & \textbf{NW} & \textbf{MZ} & \textbf{TC} &  \textbf{WB} & \textbf{AVG}  \\
% \hline
  
% \textbf{BERT-rnd} & $ 46.5 $ &  $ 48.5 $ & $ 42.1 $ & $ 36.2 $ & $ 32.5 $ & $ 30.7 $ & $ 39.4 $ \\
% \textbf{BERT-rnd-pad} & $ 50.2 $ &  $ 50.3 $ & $ 45.9 $ & $48.7 $ & $ 31.2 $ & $ 26.3 $ & $ 42.1 $ \\
% \textbf{BERT} & $ 50.9 $ &  $ \textbf{55.1} $ & $ 45.2 $ & $ 47.1 $ & $ 32.8 $ & $ \textbf{34.1} $ & $ 44.2 $ \\
% \textbf{BERT-pad} & $ \textbf{55.5} $ &  $ 54.7 $ & $ \textbf{49.4} $ & $ \textbf{53.7} $ & $ \textbf{33.2} $ & $ 30.4 $ & $ \textbf{46.2} $ \\
% \hline
% \end{tabular}
% \end{adjustbox}
% \caption{NER - AUC}\label{tab:ner-auc}

% \end{table}

Table~\ref{tab:main-results} presents our main results. 
In Figure~\ref{fig:sa-ner-main}, we present the results of two representative setups for each task, with a breakdown to iterations.
% As our results indicate, methods that leverage domain knowledge in the process of data annotation improve upon those that do not.
As our results indicate, methods that integrate DA and AL, which is a novel contribution of this paper, performs best on both tasks.


For both tasks, Figure~\ref{fig:sa-ner-main} demonstrates the effectiveness our methods compared to \rbert{} (AL, DA, and their combination) across (almost) all active learning iterations.
In NER, the trend is clear, AL methods improve upon random annotation methods (e.g., \bert{} compered to  \rbert), and DA approaches improve upon non-DA approaches (e.g., \rdt vs. \rbert). Importantly, we observe a complementary effect when combining AL and DA, with \tapad{} and \dt{} outperforming all other methods, with an average improvement of $2.0\%$ and $1.2\%$ (AUC) compared to \bert{} (their AL-based baseline) and an average improvement of $4.2\%$ and $4.6\%$ (AUC) compared to \rtapad{} and \rdt{} (their DA baselines). For SA, while UDA methods prove to be highly efficient (e.g., consider \rbert{} vs. \rdt), AL gains are inconsistent. On the one hand, \smoothing{} and \dropout{} improve \rbert{} by $0.6\%$ and $0.8\%$, respectively, on average. On the other hand, \rbert{} and \bert{} are equivalent. Nevertheless, it is \select{} and \dt{}, which combine AL and DA, that perform best, with an average improvements of $7.3\%$ and $3.6\%$, respectively, on top of the vanilla baseline, \rbert. 

Finally, we notice a limitation of the \select{} method, exhibiting dramatic performance drop in the NER setups. We analyze this behaviour in \S\ref{sec:ablation}.






 




% \paragraph{The effect of confidence-based AL} 
% As shown in Table~\ref{tab:main-results}, confidence-based approaches are not always effective. These methods prove highly efficient for NER setups, with an average improvement of $4.8\%$ (AUC) compared to identical models that rely on random data selection (e.g., when comparing BERT to BERT-rnd). But surprisingly, in sentiment analysis, there seems to be no benefit in applying confidence-based AL.

% \paragraph{UDA boosts AL}
% Intuitively, leveraging massive unlabeled data in low resource setups is promising \citep{DBLP:journals/corr/abs-2006-08671}, especially when dealing with domain shift scenarios. Indeed, our results demonstrate the effectiveness of applying UDA-based algorithms in the proposed setting. \dt and \dann (both representatives of UDA approaches) utilize additional unlabeled data from the source and target domains to adapt the model representations effectively. Overall, \dt, the strongest representative of this group, outperforms all common active learning (\S~ref{sec:basic-al}) across all sentiment setups and in 4 out of 6 NER setups.

% \paragraph{Reducing annotation pool with TAPAD}
% Our proposed setup introduces a new aspect of the AL system. It raises whether the domain signal can leverage the annotation process and lead to a better generalizing algorithm. Interestingly, our results indicate that \tapad, which reduces the annotation pool to include only data from the closest domain, significantly improves downstream performance. In NER, \tapad is the best performing algorithm, outperforming the second-best performing model by $0.7\%$ on average. Furthermore, for sentiment analysis, \tapad exceeds the standard active learning algorithms by (at least) $1.9\%$ on average. We hope that these results will encourage readers to consider the domain signal when establishing an AL system.



==> Eyal_Yftah - Active Learning for unsupervised DA/6.conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}
This paper presents a new challenging learning setup where annotating data from the desired target domain is not feasible, and annotating data from available source domains is costly. 
% We experimented with various prominent approaches within this setting, mainly from the active learning and domain adaptation algorithm families and show that combining the two yields the best performance.  
We experimented with various prominent approaches within this setting, mainly from the active learning and domain adaptation algorithm families. We presented novel ways of combining the two, yielding the best performance.
% We hope our findings will encourage further research on this setup, as our results are preliminary, and we believe it's a common setup for real-world applications that should get more attention from academic researchers.
We hope our findings will encourage further research on this setup, which we believe is common for real-world applications and should get more attention from the research community.




==> Eyal_Yftah - Active Learning for unsupervised DA/7.limitations.tex <==





\section{Limitations}
\label{sec:limitations}




\paragraph{Future algorithmic solutions}
As mentioned in previous sections, we introduce a challenging setting for domain adaptation from scratch. Yet, we consider the algorithmic solutions proposed in this paper as an initial attempt. We focused on the intersection of active learning and domain adaptation and introduced novel algorithms that integrate both, while other approaches are also valid for the suggested setting. For instance, one can introduce self-training methods, apply low resource algorithms (zero-to-few shot learning), and perhaps consider combining these approaches with the ones we present in this work. We hope to inspire future work in the intersection of domain adaptation and training algorithms from the early production stages.


\paragraph{Inconsistent performance by the \select{} method}
We notice an interesting behavior of the \select{} algorithm, which performs well on SA (on average, outperforming all other models by more than $3.7\%$) while exhibiting a dramatic performance drop in NER setups. Such inconsistent behaviour across tasks, unless understood, may dissuade future implementation of this method. Thus, in \S\ref{sec:ablation}, we provide an extensive analysis of the \select{} algorithm behaviour across different tasks.


